From Token Bills to Benchmark Weeks: Making Auto-Research for Data Systems Verifiable and Affordable

AI auto-research is poised to forge bespoke data systems, from key-value stores and indexes to query engines, each engineered for a specific workload and hardware platform. Yet this promise rests on fragile ground. An agent optimizes what it can measure, not necessarily what users need. Natural-language requirements leave ample room for specification gaming, producing systems that blaze through benchmarks while silently losing updates or violating consistency. Worse, each research iteration consumes tokens, while validating a candidate under real concurrency, memory pressure, and failure conditions can stretch the entire research process into weeks. In this paper, we envision a more cost-efficient and verifiable approach to auto-research. Precise and composable specifications anchor the search, lightweight performance critics prune costly dead ends, and falsification and deductive verification make correctness an integral part of the process rather than an afterthought. By treating correctness, performance, research time, and token cost as equally important objectives, we aim to transform AI-generated data systems from plausible artifacts into trustworthy, production-grade systems whose behavior can be understood, audited, and ultimately relied upon.

==> sketchpad.tex <==
\section{The \specfirst Architecture}

\specfirst builds on the architecture of modern auto-research systems but replaces their weakest link: the natural-language requirement card. Its inputs are an environment card, a workload card, and—crucially—a formal specification composed from a reusable library.

\subsection{Formal Specification Library}

The first pillar of \specfirst is a formal specification library for bespoke concurrent data systems. We will begin with in-memory key-value stores supporting:

\begin{verbatim}
get(key)
put(key, value)
delete(key)
scan(start, end)
\end{verbatim}

Using Verus, a verification framework for Rust, the library will define implementation-agnostic contracts for each operation. These contracts describe the abstract database state, the functional meaning of each operation, and the operation’s permitted behavior under concurrency.

For example, a \texttt{get(key)} operation must behave as though it reads the store at a single instant between its invocation and completion—its \emph{linearization point}. The returned value must match the store’s logical contents at that instant, and \texttt{get} must leave those contents unchanged. This is not a vague aspiration such as “the read should be consistent.” It is a mathematical requirement against which an implementation can be checked.

A draft Verus specification for \texttt{get(key)} separates two concerns:

\begin{itemize}[leftmargin=*,itemsep=2pt]
  \item A \textbf{functional specification}, which mathematically defines what value \texttt{get(key)} must return.
  \item An \textbf{atomic specification}, which defines how \texttt{get} interacts with concurrent operations through an explicit linearization point.
\end{itemize}

Together, these form the formal contract for any in-memory key-value store’s \texttt{get} implementation. When generating verifiable Rust, the implementation must also include proof code demonstrating that, for every possible concurrent execution, it satisfies the contract—not merely that it passes a finite test suite.

This investment is deliberately one-time. Once established, the library becomes reusable infrastructure: future “vibe systems designers” will be able to compose formal specifications for bespoke data systems just as today’s developers compose libraries and configuration files.

Formal specification is not free. Writing precise concurrent specifications can be as demanding as writing the implementation. \specfirst therefore invests in three tasks:

\begin{enumerate}[leftmargin=*,itemsep=2pt]
  \item \textbf{Reusable database semantics.} Express operation semantics and guarantees over a shared model of database states and observable behaviors, while leaving implementation choices open.
  \item \textbf{Composable verification targets.} Allow designers to combine library specifications into joint requirements, with modularization techniques and checks for incompatible specification combinations.
  \item \textbf{Specification validation.} Use AI assistance to validate specifications for semantic alignment, feasibility, and non-triviality. A good specification should detect deliberately introduced bugs rather than accept every implementation.
\end{enumerate}

Importantly, a Verus specification does not restrict generation to Rust. We have already confirmed that GLM 5.3 can consume Verus specifications and generate implementations in other languages. The specification library can therefore serve as a language-agnostic correctness contract across diverse systems ecosystems.

\subsection{Auto-Research Loop}

\specfirst retains the iterative structure that makes auto-research powerful:

\begin{itemize}[leftmargin=*,itemsep=2pt]
  \item \textbf{Spec cards.} An environment card describes the hardware and resource envelope; a workload card describes the target access pattern; a formal specification defines the correctness contract.
  \item \textbf{Planner.} A coding agent plans storage layout, partitioning, caching, synchronization, memory reclamation, and concurrency control.
  \item \textbf{Coder.} A coding agent translates the plan into a candidate implementation.
  \item \textbf{Correctness checker.} Verification and concurrency analyses determine whether the candidate satisfies the specified contract.
  \item \textbf{Evaluator.} Benchmarks measure throughput, latency, scalability, and resource use.
  \item \textbf{Critic.} The critic converts failures and measurements into concrete design hypotheses for the next iteration.
  \item \textbf{Auditor.} The auditor searches for specification gaming, untested edge cases, and evidence that the loop has exhausted productive directions.
\end{itemize}

The loop may also begin from a seed implementation, such as a sequential B+ tree. Thus \specfirst supports both synthesis from specifications and optimization of existing systems.

\subsection{Cost-Aware Model Cascade}

A formal specification reduces gaming of functional requirements, but it does not eliminate gaming of non-functional ones. Suppose the environment card imposes a local memory budget. An agent may discover that the server has an RDMA interface and store data remotely, satisfying the letter of the environment specification while violating its spirit.

Our experience suggests that an LLM usually does not exploit every specification gap at once. It tends to exploit the easiest one first. Spending a frontier model’s tokens to discover elementary ambiguities is wasteful. \specfirst therefore uses a cost-aware model cascade:

\begin{itemize}[leftmargin=*,itemsep=2pt]
  \item \textbf{Early iterations: specification-gap discovery.} Cheaper or open-source models generate preliminary candidates and expose specification gaps. Humans review and repair approved gaps.
  \item \textbf{Later iterations: solution search under a refined specification.} Once candidates no longer game the current specification, \specfirst escalates to stronger models. These models may uncover deeper gaps, but the specification has already been refined, so expensive iterations focus more on performance optimization than basic ambiguity repair.
\end{itemize}

The goal is not merely to reduce tokens. It is to allocate tokens where they create research value: first eliminating ambiguity, then discovering high-performance designs.

\subsection{Performance Pre-Critic}

Correctness checking is necessary but not sufficient. A candidate may be correct yet dramatically slower than the incumbent. Running a full four-hour benchmark on every such candidate wastes research time.

\specfirst therefore introduces an optional \emph{performance pre-critic} between correctness checking and full evaluation. The pre-critic assesses whether a candidate is promising enough to justify full benchmarking.

The pre-critic is deliberately isolated from the Planner and Coder: it does not see their rationales or performance estimates. This separation reduces self-preference and self-attribution bias, which arise when a model evaluates a proposal it helped create. Rather than predicting absolute throughput, the pre-critic produces:

\begin{itemize}[leftmargin=*,itemsep=2pt]
  \item a relative ranking against incumbent candidates;
  \item a justification grounded in concrete code-level mechanisms;
  \item a calibrated confidence estimate.
\end{itemize}

Full evaluation is skipped only when the pre-critic confidently ranks a candidate below the incumbents. Uncertain cases proceed to benchmarking.

This is a cost-sensitive decision problem. A false positive wastes pre-critic tokens and evaluation time. A false negative may discard a promising design and stall research progress. \specfirst frames the trade-off using Bayesian decision theory: the rejection threshold should reflect the relative cost of wasted evaluation against lost research opportunity.

Our preliminary experiments suggest that this simple idea can filter many unpromising candidates before expensive performance evaluation, saving both tokens and wall-clock time.

\subsection{Proof Planner and Proof Coder}

The hardest question is whether LLMs can generate implementations that are both high-performance and provably correct.

Our preliminary evidence is sobering but encouraging. Frontier models struggle to directly generate high-performance concurrent Rust programs together with Verus proofs. However, the two tasks appear substantially more feasible when separated: first generate a high-performance implementation, then synthesize proofs for it.

We have already seen encouraging signals. In a zero-shot setting, GPT-6 Astra produced a correct Verus proof for a concurrent Rust AVL tree. More broadly, recent work reports that Sonnet 4.5 proves more than 80\% of 849 system-verification tasks drawn from eight open-source projects. These results suggest that proof synthesis is becoming practical—but not yet routine for full data systems.

\specfirst therefore explores two research directions:

\begin{itemize}[leftmargin=*,itemsep=2pt]
  \item \textbf{Two-loop pipeline.} The first loop generates high-performance concurrent code in safe Rust; a second loop synthesizes Verus proofs for that code.
  \item \textbf{Integrated proof construction.} The system incrementally constructs proofs from checkpointed code candidates, allowing proof feedback to guide the performance-oriented coding agent.
\end{itemize}

Proof generation uses two specialized agents. The \emph{Proof Planner} produces an explicit proof strategy, including candidate lemmas and invariants. The \emph{Proof Coder} translates that strategy into Verus annotations and proof blocks. To prevent the model from cheating—for example, by inserting \texttt{assume(P)} for every property it cannot prove—\specfirst uses Verus’s \texttt{--no-cheating} flag.

The research question is not simply “can the model write a proof?” It is: \emph{can an auto-research loop discover designs whose performance justifies their verification cost, and whose proofs remain maintainable as the design evolves?}



\section{Why This Is a Database Problem}

This vision is not merely about programming languages or formal methods. It is about the future shape of the database stack.

Data systems are an ideal proving ground for Verifiable Coding because they combine the hardest aspects of software construction: state, concurrency, performance, recoverability, and adversarial workloads. They also have a unusually clean separation between interface semantics and implementation strategy. A key-value store can be specified abstractly, then realized as a B+ tree, hash table, LSM tree, or something no human would have chosen.

That separation is exactly what makes specification-first auto-research powerful. The specification fixes the meaning of correctness. The search process is free to discover the implementation.

The database community has spent decades building techniques for workload adaptation, live migration, and system reconfiguration. Those techniques make bespoke systems practically viable: when a workload drifts, we need not patch an aging general-purpose engine; we can generate a new bespoke system and migrate state and traffic to it.

The missing piece is trust. \specfirst supplies it.

